Grasping AI: experiential exercises for designers

Artificial intelligence (AI) and machine learning (ML) are increasingly integrated into the functioning of physical and digital products, creating unprecedented opportunities for interaction and functionality. However, there is a challenge for designers to ideate within this creative landscape, balancing the possibilities of technology with human interactional concerns. We investigate techniques for exploring and reflecting on the interactional affordances, the unique relational possibilities, and the wider social implications of AI systems. We introduced into an interaction design course (n=100) nine 'AI exercises' that draw on more than human design, responsible AI, and speculative enactment to create experiential engagements around AI interaction design. We find that exercises around metaphors and enactments make questions of training and learning, privacy and consent, autonomy and agency more tangible, and thereby help students be more reflective and responsible on how to design with AI and its complex properties in both their design process and outcomes.

==> InterviewQuestions.tex <==
\section{Interview Structure and Questions}
\subsection{Questions to Students}

\textbf{About the methods cards (5 mins )}

Why did you select these methods? Can you elaborate on the expectations you had in selecting these?
What did you find useful from these methods ? What was not so useful?
Did you look at the related example projects or literature? If so, was it helpful?
Did you read the background for the method, and was it helpful?
Did you follow the method exactly, or did you adapt/appropriate it to your particular project?
Did one method support the other? Was the ordering important? Were there particular synergies?

\textbf{About the methods in relation to the design concept (5 mins)}

Would you say these methods help you to develop your concept further?  Would you say your concept improved? In which way?
Here is the drawing that you made before and after doing the methods. What would you say are the important differences between them? Was that due to a particular thing that happened through doing a method?
What was the feeling of the group after using these methods? Would you say the group feels now more equiped in designing with AI in your project after the workshop?

\textbf{About  AI qualities  as a design resource (around 3 mins per section)}

\textbf{Affordances:}
What aspects or qualities of AI became more apparent present that you were not considering before?
Some methods asked you to role-play AI, or draw a diagram of the system. Do you think this way of engaging with AI helped to understand AI in a different way? Why?

\textbf{Relations:}
Do you think the workshop helped you with considering AI as something other than just a tool?
Did the methods help you consider the AI in your project as part of a broader network of relationships? What new relations did it uncover?

\textbf{Wider implications:}
Did the methods make you think more critically about the possible broader implications and challenges of your project?  In which way?
Did the methods help you to consider how interactions might change over time?

\textbf{Final reflections (5 mins)}

Overall, did the workshop contribute to developing a new understanding of designing with and for AI?
Have you thought about using another of the methods in your own process?
Do you have any final reflection or questions?

\subsection{Questions for coaches}

\textbf{Warm up: }
How are your students/ teams progressing in the course? What can you say about their general understanding of designing with/ for AI?
How comprehensive do you feel is your understanding of AI and its use in design?
Did you have previous research/practice experience with AI and design?

\textbf{Consider for each group: }
How much did you discuss AI with them, as opposed to general interactive prototyping? Was there a significant engagement with AI in the coach meetings?
If you look at the work before and after the workshop, did you feel that the methods workshop helped the students? In what way?
Did the students engage with the particular qualities of AI (e.g. uncertainty, training, data use) a) before the workshop, b) after the workshop?
Did the students think about their project as a tool, or as part of a wider network of relations a) before the workshop, b) after the workshop
Did the students think critically about the implications of their project (social shaping, change over time, privacy etc.) a) before the workshop, b) after the workshop
Did you notice  changes  due to any particular  method reflected in the progress and development of any of the student challenges?



==> figures/method_usage.tex <==

\begin{table}
\begin{center}
\caption{Name, key references and description of each method, along with the number of groups who used it and the average score for clarity. Yellow dots ({\color{myOrange}\CIRCLE\hspace{0.001cm}}) represent the number of groups who used the method. The final four columns address perceived usefulness of the exercise for four areas: concept development, refining interactions, understanding of AI and reflection. Red dots ({\color{myRed}\CIRCLE\hspace{0.001cm}}) count the number of groups who mentioned it as being helpful for the area, with representative direct quotes in italics, summaries in normal font.}
\small
\begin{tabular}{p{1.2cm}p{4.5cm}p{0.6cm}p{0.6cm}p{1.8cm}p{1.8cm}p{1.8cm}p{1.8cm}}
\toprule
Method & Description (and inspirations) & Clarity\newline {\scriptsize(-3..3)} & Count & Concept\newline Development & Detailing \newline Interactions & Understanding AI & Reflection \\
\hline
Uncertain Inter\-actions & Look through the state diagram of your interaction; for each change of state, imagine replacing it with probabilistic, uncertain or in-between outcomes (\cite{bowler2022ExploringUncertainty} \cite{benjamin2021MachineLearning}) & 1.1 & \numUsesN{7} & \numUses{5} \qt{p24}{make it more concrete}, \qt{p6}{a screen to show why...}& \numUses{6} \qt{p7}{interaction in detail}, \qt{p24}{prepared for difficult conversations} & \numUses{2} \qt{p16}{better prepared for [] error interactions} & \numUses{2} \qt{p16}{reconsider intentions}\\
\hline
Be the ML & From a live view of the data inputs to your system, try to perform the activity yourself, then explain what you’re doing to someone else (\cite{devendorf2015BeingMachine} \cite{scurto2021PrototypingMachine}) & 2 & \numUsesN{1} & \numUses{1} \qt{p24}{gave us an overview}&  & \numUses{1} \qt{p24}{listening to human emotions is hard} &\\
\hline
Poor Datasets  & Iteratively remove examples from your dataset, decreasing diversity of the input and retraining the model until something problematic happens. (\cite{elwes2019Zizi} \cite{buolamwini2018GenderShades}) & not used & not used  & & & & \\
\hline
Thing Ethno\-graphy of AI Systems &  Collect data from the perspective an object in your system; use it make sense of the situation around the device; what does it experience that you didn’t know? Who does it interact with? (\cite{giaccardi2016ThingEthnography} \cite{murray-rust2019EntangledEthnography} & 2 & \numUsesN{2} & \numUses{2} \qt{p22}{the journey of the object outside the interaction} & \numUses{2} \qt{p22}{react to being held} & \numUses{1} \qt{p22}{[camera] viewpoint was not suitable} & \\
\hline
Conver\-sations with AI &  Choose one of the AI powered objects in your interaction. One team member plays the character of the object, and others carry out an interview with that object. (\cite{nicenboim2020MoreThanHumanDesign} \cite{reddy2021MakingEveryday}) & 2.2 & \numUsesN{5} & \numUses{3} \qt{p2}{takes state of mind into account}, \qt{p3}{give AI a purpose} & \numUses{3} move from passive to active [p10], feel-good to good [p2] & \numUses{2} \qt{p3}{AI cannot have the same experience as you}, \qt{p2}{sensitizer} & \numUses{1} parts are separated, importance of roles (p10) \\
\hline
Metaphor Shifts & Think about the metaphors  use in describe your system, then think about designing purely for the metaphor; change metaphors and try again (\cite{murray-rust2022MetaphorsDesigners,lockton2019NewMetaphors,alves-oliveira2021CollectionMetaphors} ) & 1.8 & \numUsesN{14} & \numUses{11} \qt{p16}{role and character}, \qt{p7}{different perspectives} & \numUses{6} \qt{p3}{find a way to initiate negotiation}, \qt{p23}{gets a character}& \numUses{3}\qt{p18}{AI needs to be specific}, \qt{p3}{AI as a protective agent} & \numUses{5} \qt{p16}{how that intention has manifested itself into the concept} \\
\hline
Roleplaying AI\newline Networks &  Play an object, system or human role and collaboratively act out the interaction. Discover new actors, negotiations,  relationships and interaction details (\cite{pschetz2019AutonomousDistributed} \cite{reddy2020EncounteringEthics}) & 1.2 & \numUsesN{5} & \numUses{4} \qt{p12}{new agents and interactions}, \qt{p13}{better clarity} & \numUses{4} \qt{p13}{draw out interactions}, \qt{p27}{elaborate on context} & \numUses{1} \qt{p13}{understanding of specific [technical] elements} & \numUseAlign none reported \\
\hline
Resisting/ Subverting AI &  Recognise and act out moments in the interaction where someone might subvert the interaction; look for design opportunities (\cite{lupetti2020SubversiveCitizen} \cite{disalvo2015AdversarialDesign}) & 1.0 & \numUsesN{3} & \numUses{3} \qt{p18}{exploring new ideas}, \qt{p8}{chances to be misused} & \numUses{3}  \qt{p28}{things we knew but never wrote down}, \qt{p8}{criticality}& \numUses{1} adversarial sensing (p8) & \numUses{1} \qt{p8}{think critically}\\
\hline
Meaningful Human Control & Brainstorm places where the interaction might go wrong; rather than trying to fix it, figure out who or what is responsible and how they might be supported in setting their moral boundaries. (\cite{siebert2022MeaningfulHuman}) & 1.0 & \numUsesN{7} & \numUses{5} \qt{p19}{making our design more responsible}, \qt{p2}{Introduce [...] resistance} & \numUses{5} \qt{p25}{development of consent}, \qt{p19}{part of interactions we haven't planned} & \numUses{3} \qt{p3}{understand the richness}, \qt{p2}{mess with your moral judgement} & \numUses{2}  \qt{p21}{consider user vulnerability}, \qt{p25}{bring across critical view} \\
\bottomrule
\end{tabular}

\label{table:USAGE}
\end{center}
\end{table}



